SoK: Blockchain Technology and Its Potential Use Cases

Bitcoin's success has led to significant interest in its underlying components, particularly Blockchain technology. Over 10 years after Bitcoin's initial release, the community still suffers from a lack of clarity regarding what properties defines Blockchain technology, its relationship to similar technologies, and which of its proposed use-cases are tenable and which are little more than hype. In this paper we answer four common questions regarding Blockchain technology: (1) what exactly is Blockchain technology, (2) what capabilities does it provide, and (3) what are good applications for Blockchain technology, and (4) how does it relate to other approache distributed technologies (e.g., distributed databases). We accomplish this goal by using grounded theory (a structured approach to gathering and analyzing qualitative data) to thoroughly analyze a large corpus of literature on Blockchain technology. This method enables us to answer the above questions while limiting researcher bias, separating thought leadership from peddled hype and identifying open research questions related to Blockchain technology. The audience for this paper is broad as it aims to help researchers in a variety of areas come to a better understanding of Blockchain technology and identify whether it may be of use in their own research.

==> sections/criteria.tex <==
% !TEX root = ../main.tex

\section{Lessons Learned (Scott/Ben)}

What was missing in the graph?
	Off-chain stapling
	Anonymity
		MPC
		Functional encryption
	Authenticated data structure

Terminology

Normative vs. technical properties
	public participation is a huge normative property. Not gauntleted to be in a Blockchain.
	There are risks of thinking they are the same
		Using blockchain assuming you get normative properties, not just technical properties
		Get saturated on normative properties, ignore the technical properties
	Diffused trust vs. trustfulness
	Decentralization
		Governance and communication are required to be decentralized
		Disintermediation is normative, and may or may not be part of a Blockchain
			There are always intermediaries. Decentralization limits their power.



How do we know which use cases are good fits for Blockchain?
Criteria
	1) Decentralized governance (*)
	2) Auditability
	3) Resiliency	
Is there a question tree we can create?
